Breaking the Limits of Message Passing Graph Neural Networks

Since the Message Passing (Graph) Neural Networks (MPNNs) have a linear complexity with respect to the number of nodes when applied to sparse graphs, they have been widely implemented and still raise a lot of interest even though their theoretical expressive power is limited to the first order Weisfeiler-Lehman test (1-WL). In this paper, we show that if the graph convolution supports are designed in spectral-domain by a non-linear custom function of eigenvalues and masked with an arbitrary large receptive field, the MPNN is theoretically more powerful than the 1-WL test and experimentally as powerful as a 3-WL existing models, while remaining spatially localized. Moreover, by designing custom filter functions, outputs can have various frequency components that allow the convolution process to learn different relationships between a given input graph signal and its associated properties. So far, the best 3-WL equivalent graph neural networks have a computational complexity in $\mathcal{O}(n^3)$ with memory usage in $\mathcal{O}(n^2)$, consider non-local update mechanism and do not provide the spectral richness of output profile. The proposed method overcomes all these aforementioned problems and reaches state-of-the-art results in many downstream tasks.

==> BeyondWL1.tex <==
\section{MPNN Beyond 1-WL}

To create a Graph MPNN which is able to produce all sentences in $\mathcal{L}_1$, here we proposed model and its proof in following theorem.

\begin{theorem}
\label{th:th1}
A MPNN following the update schema given by 
\begin{equation}
  \label{eq:ml1}
  \scriptstyle
  H^{(l+1)}=\sigma\left( H^{(l)}W^{(l,1)}+AH^{(l)}W^{(l,2)} + H^{(l)}W^{(l,3)}\circ H^{(l)}W^{(l,4)}  \right)
\end{equation}
where $W^{(l,s)}$ are trainable parameters can produce every possible sentences in $ML(\mathcal{L}_1)$ for undirected graph adjacency $A$ with monochromatic edges and nodes. Thus, such a MPNN called $GNNML_1$ is as powerful as 1-WL test.
\end{theorem}


The new representation of the node consists of three parts. These are previous layer representation's linear transformation, sum of connected node's previous layer's representations linear transformation and finally two different linear transformations of previous layer's node representation's elements-wise multiplication.

Although, this model provable has the same power with 1-WL so do GIN in order to distinguish two non-isomorphic graphs, because of third part of the update schema in Eq.\eqref{eq:ml1}, it can produce multiplication of features on each layer, its node representation is richer, thus it would be more powerful in order to count substructures as we show in the result.

Using theoretical researches in \cite{geerts2020expressive} by giving Remark~\ref{rm:rm2},\ref{rm:rm3} and \ref{rm:rm5}, we need a model which can produce different output than $\mathcal{L}_1^+$ language to have more powerful model than 1-WL. %Although Chebnet can go a little further beyond 1-WL (for the pair of graphs whose maximum eigenvalues are not the same), it has less empirical advantage as we show in the result section.
According to Remark~\ref{rm:rm3} and Remark~\ref{rm:rm5}, trace ($tr$) and element-wise multiplication ($\odot$) operation make the model go further than 1-WL. 

In order to show the impact of trace operation, we can use 1-WL equivalent Decalin and Bicyclopentyl graphs in Figure~\ref{dec_bicyc}. It is easy to show that $tr(A_G^5)=0$ but $tr(A_H^5)=20$ where these results are number of 5-length closed walk. Thus, if the model has ability to apply trace operator over some power of adjcency, it can easily distinguish these two graphs. The computational details are found in Appendix~\ref{app2}. 

\begin{figure}[ht]
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.5\columnwidth]{figures/cospectral_graphs.jpg}}
\caption{Cospectral and 4-regular graphs from \cite{van2003graphs} are $\mathcal{L}_1$ and $\mathcal{L}_2$ equivalent.
}
\label{cospect}
\end{center}
\vskip -0.2in
\end{figure}

On the other hand, trace operator is not enough for cospectral graphs, since the cospectral graphs, such as in Figure~\ref{cospect}, have the same number of closed walk of any length \cite{geerts2020expressive}(Proposition5.1). But using element-wise multiplication, we can write a sentences as $e(A)={\bf1}^{\top}f((A\odot A^2)^2{\bf1})$  where $f(x)=x^2$ for given vector, its output becomes $e(A_G)=6032$ and $e(A_H)=5872$ for given two graphs in Figure~\ref{cospect} respectively, thus it can distinguish these two graphs. The calculation details can be found in Appendix~\ref{app3}.

As we have seen, the model which enriched by element-wise multiplication and trace operator can go further than 1-WL test power. However, these operations needs to keep power of adjacency explicitly and multiply these dense power matrix to each other by matrix or element-wise multiplication which is what higher order GNNs do such as \cite{maron2019provably, 123lehmango}. But, MPNN cannot calculate the power of given adjacency explicitly. Instead, it multiplies the last representation of the nodes by sparse adjacency or any sparse convolution supports $C$ in Eq.\eqref{eq:mpgnn} for every layer. More precisely, if the given node fetaures are $H^{(0)}={\bf1}$, MPNN can calculate, for instance, $C^3{\bf1}$ by 3 layered MPNN in a way of $C.(C.(C.{\bf1}))$ but not in a way of $(C^3){\bf1}$. Since MPNN does not keep $C^3$ explicitly, it cannot take its trace or multiply element-wise to another power of support. This is the disadvantage of MPNN. On the other hand, this is the reason why MPNN needs just linear time and memory complexity which makes it advantageous.

One solution might be designing graph convolution supports by the point-wise multiplication of some power of adjacency matrix and desired receptive field such as $C^{(s)}=M\odot A^s$ where $M$ masks the component of the power matrix and keep the convolution support sparse. For example, we can use $M=A+I$ for maximum 1-length receptive field. Even though this model cannot calculate all possible point-wise multiplication between all possible matrices, but at least it can produces any sentence in a form of $(M\odot A^s)^l$ where $l \in [l_{max}]$ is the number of layer and $s \in [s_{max}]$ is the predefined power of convolution supports. In this proposition, we need to define receptive field mask and how many power of adjacency should be used in prepossessing step. However, we cannot know initially that what power of adjacency matrix is necessary for particular problem. One selection would be tuning it as hyperparameter of the model. Another problem of this approach is that having power of adjacency makes the convolution supports consist of higher number which needs to be normalized.

%Using adjacency or laplacien cannot change the expressive power of the model. Because the laplacien can be written by operation in $\mathcal{L}^+$ by adjacency, it's expressive power is not different than adjacency.
To overcome these mentioned problems, we propose to design MPNN's convolution supports by function of normalized laplacien's or adjacency's eigenvalues in spectral domain which literally can be written power series of graph laplacien or adjacency. We call this proposed model GNNML3.

\begin{theorem}
\label{th:th4}
GNNML3's convolution supports set to ;
\begin{equation}
  \label{eq:th4eq11}
  C'^{(s)}=U diag(\Phi_s(\lambda))U^{\top}
\end{equation}
where $\Phi_s(\lambda)=exp(-b(\lambda-f_s)^2)$, $f_s\in [\lambda_{min},\dots,\lambda_{max}]$ is a scalar design parameter of each convolution support and $b >0$ is a general scalar design parameter, 
%, and $M$ is receptive field mask, 
consist of linear combination of all powers of graph laplacien (or adjacency) as follows;
\begin{equation}
  \label{eq:th4eq12}
  C'^{(s)}=\alpha_{s,0}L^0 +\alpha_{s,1}L^1+  \dots +\alpha_{s,n}L^n
\end{equation}
where $\alpha_{s,i}=\frac{\Phi_s^{(i)}(0)}{i!}$ are scalar coefficients.
\end{theorem}

Since each matrix's design parameters ($f_s$) are different, each $C'^{(s)}$ in Eq.\eqref{eq:th4eq12} consist of different linear combination of power series of graph laplacien (or adjacency). Thus we can learn necessary power of laplacien (or adjacency) and also produce their point-wise multiplication by 
\begin{equation}
  \label{eq:learnsup}
  C=M \odot mlp_{4}\left (mlp_{1}(C') | mlp_{2}(C') \odot mlp_{3}(C')\right )
\end{equation}
where $C'=[C'^{(1)}|\dots|C'^{(s)}] \in \mathcal{R}^{n\times n \times S}$ is stacked initial convolution supports on 3-th dimension, $mlp_{k}(.)$ is a trainable model performed on 3-th dimension on given tensor, $C=[C^{(1)}|\dots|C^{(S)}] \in \mathcal{R}^{n\times n \times S}$ sparsified convolution support by defined receptive field mask $M$. The forward calculation of one layer MPNN becomes as follows;
\begin{equation}
  \label{eq:ml2}
  \scriptstyle
  H^{(l+1)}=\sigma\left( \sum_s(C^{(s)}H^{(l)}W^{(l,s)}) | H^{(l)}W^{(l,1)}\odot H^{(l)}W^{(l,2)}  \right)
\end{equation}   

There are infinitly many selection of $\Phi_s(\lambda)$ which makes the convolution support written by power series of graph laplacien (or adjacency). However, by our selection, each convolution is sensitive on each band of spectrum ($f_s$) by given bandwidth ($b$) thus it is able to learn relations if the solution depends on spectrum of signal on graph.

Algorithm~\ref{alg:preproces} shows how to calculate the initial convolution supports ($C'$). Since we calculate the supports for valid indices in receptive field mask (where $M_{i,j}=1$) we can see $C'$ as extracted edge features where the edge indexes are defined by $M$. In application we use a function $sparse2vec: \mathcal{R}^{n \times n} \rightarrow \mathcal{R}^{m}$ that converts the sparse matrix to vector by just keeping the components on valid indices of mask.

\begin{algorithm}[tb]
  \caption{GNNML3's Preprocessing Step}
  \label{alg:preproces}
\begin{algorithmic}
  \STATE {\bfseries Input:} adjacency $A \in \mathcal{R}^{n \times n}$, receptive field mask $M \in \{0,1\}^{n \times n}$, number of supports $S \in \mathcal{N}$, frequency responses function of each support $\Phi_1(\lambda) \dots \Phi_S(\lambda)$
  \STATE {\bfseries Output:} extracted edge features $C' \in \mathcal{R}^{m \times S}$
  \STATE Set basis matrix: $B=I-D^{-1/2}AD^{-1/2}$ or $B=A$.
  \STATE Eigendecomposition: $Udiag(\lambda)U^{\top}=B$
  \FOR{$s=1$ {\bfseries to} $S$}
  \STATE $C'_{:s}=sparse2vec\left( M \odot (U diag(\Phi_s(\lambda))U^{\top})\right)$
  \ENDFOR
\end{algorithmic}
\end{algorithm}

Algorithm~\ref{alg:proposed} shows the forward calculations of the model for just one graph. To make the representation as simple as possible, we prefer to use tensor representation in Eq.\eqref{eq:learnsup}.
However, in application in Algorithm~\ref{alg:proposed}, we just apply $mlp_{k}(.)$ on to the valid indices defined by receptive field mask $M$. Thus, $C,C' \in \mathcal{R}^{m \times S}$ where $m$ shows number of valid indices in $M$ and $mlp_{k}(.)$ applies on columns of $C'$. Beside, we use a function $vec2sparse: \mathcal{R}^{m} \rightarrow \mathcal{R}^{n \times n}$ which converts the vector to the sparse convolution support according to given mask $M$.

The limits of proposed method is the same with 3-WL (or 2-FWL) test. For instance, strongly regular graphs which can be defined by 3 parameters, one shows the degree of the nodes, one shows the number of common neighbours of adjacent node pairs, another shows the number of common neighbours of non-adjacent node pairs. %Thus if the graph is strongly regular, all connected node pair should have the same number of common neighbours so do non-adjacent pairs as well. 
These graphs are provably known 3-WL equivalent \cite{arvind2020weisfeiler}. In Appendix~\ref{app4} a strongly regular graphs pair and result of a sample sentence in $\mathcal{L}_3$ can be found. 

\begin{algorithm}[tb]
  \caption{GNNML3's Forward calculation}
  \label{alg:proposed}
\begin{algorithmic}
  \STATE {\bfseries Input:} extracted edge features
  $C' \in \mathcal{R}^{m  \times S}$, initial node feature $H^{(0)} \in \mathcal{R}^{n \times f_0}$, receptive field mask $M \in \{0,1\}^{n \times n}$, number of layer $L$, number of supports $S$
  \STATE {\bfseries Output:} new node representation $H^{(L)}$
  %\REPEAT
  %\STATE Initialize $noChange = true$.
  \FOR{$l=0$ {\bfseries to} $L-1$}
  \STATE $\scriptstyle \Tilde{C}=mlp_{l,4}(mlp_{l,1}(C') | mlp_{l,2}(C') \odot mlp_{l,3}(C'))$
  \FOR{$s=1$ {\bfseries to} $S$}
  \STATE
  $\scriptstyle C^{(s)}=vec2sparse(\Tilde{C}_{:s},M)$
  \ENDFOR
  \STATE
  $\scriptstyle
  H^{(l+1)}=\sigma\left( \sum_s(C^{(s)}H^{(l)}W^{(l,s)}) | mlp_{l,5}(H^{(l)})\odot mlp_{l,6}(H^{(l)}) \right)$
  
%   \IF{$x_i > x_{i+1}$}
%   \STATE Swap $x_i$ and $x_{i+1}$
%   \STATE $noChange = false$
%   \ENDIF
  \ENDFOR
  %\UNTIL{$noChange$ is $true$}
\end{algorithmic}
\end{algorithm}

==> GNNreview.tex <==
\section{Message Passing Graph Neural Networks}
%MPNN is one of the most general framework defining GNNs \cite{gilmer17:_neural_messag_passin_quant_chemis}. The new representation of nodes are obtained after message passing procedure between nodes. This section describes this general framework and notations.
%In this section, we briefly describe our notations and we present the general framework.% we use for Message Passing GNN, taken from \cite{balcilar2021analyzing}.

\subsection{Notations}

Let $G$ be a graph with $n$ nodes and an arbitrary number of edges. Connectivity is given by the adjacency matrix $A \in \{0,1\}^{n \times n}$ and features are defined on nodes by $X \in \mathbb{R}^{n \times f_0}$, with $f_0$ the length of feature vectors. For any matrix $X$, we used $X_i$, $X_{:j}$ and $X_{i,j}$ to refer to its $i$-th column vector, $j$-th row vector and ($i,j$)-th entry,  respectively. A graph Laplacian is given by $L=D-A$ (or $L=I-D^{-1/2}AD^{-1/2}$) where $D \in \mathbb{R}^{n \times n}$ is the diagonal degree matrix and $I$ is the identity. Through an eigendecomposition, $L$ can be written by $L=U \text{diag}(\blambda) U^T$ where each column of $U \in \mathbb{R}^{n \times n}$ is an eigenvector of $L$, $\blambda \in \mathbb{R}^n$ gathers the eigenvalues of L and $\text{diag}(\cdot)$ creates a diagonal matrix whose diagonal elements are from a given vector. We use superscripts to refer to vectors or matrices evolving through iterations or layers. For instance, $H^{(l)} \in \mathbb{R}^{n \times f_l}$ refers to the node representation on layer $l$ whose feature dimension is $f_l$.
A Graph Convolution layer takes the node representation of the previous layer $H^{(l-1)}$ as input and produces a new representation $H^{(l)}$, with $H^{(0)}=X$.

\subsection{Generalization of Spectral and Spatial GNNs}
\label{sec2.2}
Usually, GNNs are classified as either spectral or spatial in the literature \citep{wu19:_compr_survey_graph_neural_networ,chami2020machine}. Spectral GNNs rely on the spectral graph theory~\citep{OL-CHUNG-1997}. In this framework, signals on graphs are filtered using the eigendecomposition of the graph Laplacian \citep{shuman2013emerging}. By transposing the convolution theorem to graphs, the spectral filtering in the frequency domain can be defined by $x_{flt} =  U \text{diag}( \Omega(\blambda)) U^\top x$, where $\Omega(.)$ is the desired filter function which needs to be learnt by back-propagation. On the other hand, spatial GNNs consider two operators, one that aggregates the connected nodes messages and one that updates the concerned node representation.

In a recent paper \cite{balcilar2021analyzing}, it was explicitly shown that both spatial and spectral GNNs are MPNN, taking the general form% which can be generalized in the following form :
\begin{equation}
   \label{eq:mpgnn}
   H^{(l+1)} = \sigma \Big( \sum_s C^{(s)} H^{(l)} W^{(l,s)} \Big),
\end{equation}
where $C^{(s)} \in \mathbb{R}^{n \times n}$ is the $s$-th convolution support that defines how the node features are propagated to the neighboring nodes and $W^{(l,s)} \in \mathbb{R}^{f_l \times f_{l+1}}$ is the trainable matrix for the $l$-th layer and $s$-th support. 
Within this generalization, GNNs differ from each other by the design of the convolution supports $C^{(s)}$. If the supports are designed in the spectral domain by $\Phi_s(\blambda)$, the convolution support needs to be written as $C^{(s)} = U \text{diag} (\Phi_s(\blambda)) U^\top$. 
%The final layer embedding will be considered as the output of the model.

One can see that as long as $C^{(s)}$ matrices are sparse (number of edges is defined by some constant multiplied by the number of nodes), MPNN in Eq.\ref{eq:mpgnn} has linear memory and computational complexities with respect to the number of nodes. Because, the valid entries in $C^{(s)}$ that we need to keep is linear with respect to the number of nodes and thank to the sparse matrix multiplication $C^{(s)}H^{(l)}$ takes linear time with respect to the number of edges thus nodes as well. %regardless of the input output feature length ( i.e $f_l=f_{l+1}=1$). 




%% 
% \subsection{Generalization of Spectral and Spatial GNNs}
% \label{sec2.2}
% Usually, GNNs are classified as either spectral or spatial in the literature \citep{wu19:_compr_survey_graph_neural_networ,chami2020machine}.

% Spectral GNNs rely on the spectral graph theory~\citep{OL-CHUNG-1997}. In this framework, signals on graphs are filtered using the eigendecomposition of graph Laplacian \citep{shuman2013emerging}. By transposing the convolution theorem to graphs, the spectral filtering in the frequency domain can be defined by $x_{flt} =  U \text{diag}( \Omega(\blambda)) U^\top x$, where $\Omega(.)$ is the desired filter function which needs to be learnt by back-propagation. 

% On the other hand, spatial GNNs, also called MPNNs, consider an $agg$ operator, which aggregates the neighborhood nodes, and an $upd$ operator, which updates the concerned node as follows:
% \begin{equation}
%   \label{eq:spat}
%   H_{:v}^{(l+1)} = upd \Big( g_0(H_{:v}^{(l)}) , agg \Big( {g_1(H_{:u}^{(l)}): u \in \mathcal{N}(v)} \Big) \Big),
% \end{equation}
% where $\mathcal{N}(v)$ is the set of neighborhood nodes of node $v$ and $g_0,g_1:\mathbb{R}^{n \times f_l} \rightarrow \mathbb{R}^{n \times f_{l+1}}$ are some trainable models. The choice of $agg,upd,g_0,g_1$ and even $\mathcal{N}(v)$  determines the capability of model.

% {\color{blue}In a recent paper \cite{balcilar2021analyzing}, it was explicitly shown that if the two following conditions are met : 
% \begin{itemize}
%     \item spectral models are parameterized by $\Omega(\blambda)=Bw$, $B \in \mathbb{R}^{n \times s_e}$ being a function of eigenvalues $B_{k,s}=\Phi_s(\lambda_k)$, where  $k=1,\dots,n$ denotes eigenvalue index, $s=1,\dots,s_e$ denotes index of filters, $s_e$ is the number of desired filters and $w \in \mathbb{R}^{1 \times s_e}$ are trainable parameters;
%     \item spatial approaches are  defined such that $upd(x,y)=\sigma(x+y)$, where $agg$ is a sum (or a weighted sum) of the defined neighborhood node contributions and $g_i$ applies linear transformations;
% \end{itemize}
% then both approaches can be generalized in the following form :}
% \begin{equation}
%   \label{eq:mpgnn}
%   H^{(l+1)} = \sigma \Big( \sum_s C^{(s)} H^{(l)} W^{(l,s)} \Big),
% \end{equation}
% where $C^{(s)} \in \mathbb{R}^{n \times n}$ is the $s$-th convolution support that defines how the node features are propagated to the neighboring nodes and $W^{(l,s)} \in \mathbb{R}^{f_l \times f_{l+1}}$ is the trainable matrix for the $l$-th layer and $s$-th support. 
% Within this generalization, GNNs differ from each other by the design of the convolution supports $C^{(s)}$. If the supports are designed in the spectral domain by $\Phi_s(\blambda)$, the convolution support needs to be written as $C^{(s)} = U \diag (\Phi_s(\blambda)) U^\top$. 

% The final layer embedding will be considered as the output of the model. One can see that as long as $C^{(s)}$ matrices are sparse (number of edges is defined by some constant multiplied by the number of nodes), MPNN in Eq.\ref{eq:mpgnn} has linear memory and computational complexity with respect to the number of nodes regardless of the input output feature length ( i.e $f_l=f_{l+1}=1$). 



==> MNPPbeyondWL1.tex <==
\section{MPNN Beyond 1-WL}

Because of having the same memory and computational complexity and also similarity between Eq.\ref{eq:spat} and Eq.\ref{eq:wl1}, there is a consensus that all message passing GNN has equivalent power of 1-WL test. However, in this section, we theoretically show that some GNN is less powerful than 1-WL, some is strictly more powerful than 1-WL and also a way of breaking 1-WL limit to be able to have 3-WL (2-FWL) equivalent of Message Passing GNN. 

We call two graphs $G$ and $G'$ k-WL (or FWL) equivalent if they are indistinguishable by k-WL (or FWL) and shown by $G\equiv_{k-WL}G'$.
Since our analysis is limited for 1-WL and 3-WL (or 2-FWL) there is two options which are $G\equiv_{1-WL}G'$ and $G\equiv_{3-WL}G'$ (or $G\equiv_{2-FWL}G'$).

In our theoretical analysis, we consider the given two undirected graphs have the same number of featureless nodes and edges which is the most difficult case to test graph isomorphism.

\begin{theorem}
  \label{Th:th1}
Let $A,A' \in \{0,1\}^{n \times n}$ are the adjacency matrices of two undirected graphs consist of monochromatic nodes and edges. If any color of vertices $H=\sigma(A, H^{(0)}), H'=\sigma(A', H'^{(0)}) \in \mathbb{R}^n$, there is a common permutation matrix $\Pi \in \{0,1\}^{n \times n}$ which consist of single 1 in each rows and col that meets followings;
\begin{equation}
  \label{eq:th1e1}
  H=\Pi H', ~~AH=\Pi A'H',  %\rightarrow
  %\sigma(A H^{(t)})=\Pi \sigma(A'H'^{(t)}), 
  %~~ \forall t \in N
\end{equation}
the graphs are 1-WL equivalent. 

where $H^{(t)}=A H^{(t-1)},H'^{(t)}=A' H'^{(t-1)} \in \mathbb{R}^n$ is colors of vertices at iteration $t$, may be initialized by $H^{(0)}={\bf1}$.
\end{theorem}
\begin{proof}
If we simplify Eq \ref{eq:wl1} by using sum %followed by injective element-wise function
for order invariant set operator $\{.\}$, the update can be written by $H^{(t+1)} = \left( H^{(t)}~ |A H^{(t)} \right)$. For another graph, we can write it as $H'^{(t+1)} = \left( H'^{(t)}~ |A' H^{(t)} \right)$. According to definition of WL test, if two graphs are 1-WL equivalent, their node color histograms should be same at iteration $t+1$ thus, $hist\left( H^{(t)}~ |A H^{(t)} \right) = hist\left( H'^{(t)}~ |A' H'^{(t)} \right)$. If the histogram of two sets are equal, it means there is a permutation which rearrange one and get another. It means there is at least one $\Pi \in \{0,1\}^{n \times n}$ that meets  $\left( H^{(t)}~ |A H^{(t)} \right))= \Pi \left( H'^{(t)}~ |A' H'^{(t)} \right)$. Since $|$ is the concatenation operator, both parts of the equation should be equal independently under the same $\Pi$ permutation matrix. Thus , we can obtain Eq \ref{eq:th1e1}. If this constraint is met, the new color of the vertices are calculated and Eq.\ref{eq:th1e1} checks again. For new color calculation, we do not need to keep previous colors by $H^{(t)}$ and $H'^{(t)}$. Because they have the same color under the same permutation matrix by $AH^{(t)}$ and $A'H'^{(t)}$. It just have effect on elongate the color representation. Thus we can remove it as a part of relabelling process in 1-WL algorithm. The update needs to be $H^{(t+1)}=A H^{(t)},H'^{(t+1)}=A' H'^{(t)}$
\end{proof}

If the graphs are not 1-WL equivalent, at some $t$ iteration, Eq.\ref{eq:th1e1} does not meet. To compare any GNN's theoretical power with 1-WL, we should theoretically explain the constraints that GNN makes decision on equivalent, then find a situation where one concludes they are equivalent, but another not.

In order to analyse the theoretical power of GNN in terms of ability on distinguish non-isomorphic pairs of graphs, we can neglected the trainable parameters $W$ (assume $W=I$) and element-wise injective non-linearity $\sigma(.)$ (assume $\sigma(x)=x$) in Eq.\ref{eq:mpgnn}, since whatever they are, they cannot make any differences between graphs new embedding if the rest of them are the same ($H^{(t)}=\Pi H'^{(t)} \rightarrow  \sigma(W.H^{(t)})=\Pi \sigma(W.H'^{(t)})$). Thus new representation of the vertex color can be defined by $H^{(t+1)} =  \sum_s C^{(s)} H^{(t)}$ for GNN. For sake of simplicity, we can evaluate each convolution support independently for multi-support GNN case. If ever one support has ability to distinguish some pair of graphs, the model has that ability because of adding each supports embeddings to obtain final embeddings. 

\begin{theorem}
  \label{Th:thmlp}
Graph agnostic Neural Network named MLP cannot distinguish any pair of non-isomorphic graphs which can be identified by 1-WL at iteration $t>0$. Thus, MLP is strickly less powerful that 1-WL.
\end{theorem}
\begin{proof}
We can use MLP in order to make baseline if the structural information has effect to the problem target or not. In general framework in Eq. \ref{eq:mpgnn} we can define MLP by single convolution supports as it is $C^{(1)}=I$. To be equivalent according to MLP is to meet following constraint.

\begin{equation}
  \label{eq:thmlp}
  H^{(t)}=\Pi H'^{(t)}, ~~IH^{(t)}=\Pi I H'^{(t)}, ~~ \forall t \in N
\end{equation}

Since $H^{(t)}=IH^{(t)}$, actually second constraints does not say anything. It means, if the first constraint meet in Eq.\ref{eq:th1e1} but second not that 1-WL concludes that they are not isomorphic, still MLP's constraints meet (because first constraints of 1-WL is the same to both constraints of MLP) yields that MLP concludes they are isomorphic. Thus we can conclude that MLP is strictly less powerful than 1-WL. MLP can identify non-isomortphic graphs if they can be distinguishable by the given initial colors at iteration $t=0$ in 1-WL.
\end{proof}
\begin{theorem}
  \label{Th:thsage}
GraphSage which uses full sampling and mean aggregator in \cite{hamilton2017sage}, cannot distinguish any pair of non-isomorphic graphs, whose initial color is monochromatic. Thus, GraphSage is strickly less powerful that 1-WL.
\end{theorem}
\begin{proof}
In literature GraphSage method has was proposed to sample neighborhood and aggregate the neighborhood contribution by mean operator or LSTM in \cite{hamilton2017sage}. Since we restrict the method using full sampling and mean aggregator, we can define GraphSage by general framework in Eq.\ref{eq:mpgnn} while two convolution supports are identity matrix $C^{(1)}=I$ and row normalized adjacency matrix $C^{(2)}=\tilde{A}$. Theorem~\ref{Th:thmlp} shows that $C^{(1)}=I$ is nothing but just comparing initial vertex color. So we can just consider $C^{(2)}=\tilde{A}$. Thus constraints of GraphSage will be as follows;
\begin{equation}
  \label{eq:thsage1}
  H^{(t)}=\Pi H'^{(t)}, ~~\tilde{A}H^{(t)}=\Pi \tilde{A'} H'^{(t)}, ~~ \forall t \in N
\end{equation}
When we start by monochromatic vertex color as $H^{(0)}=H'^{(0)}={\bf1}$, since the row normalized adjacency meets $\tilde{A}{\bf1}=\tilde{A'}{\bf1}={\bf1}$, second constraint will always meet, even though the case where 1-WL's second constraint does not meet. %Thus we can conclude that if the GraphSage starts with monochromatic vertex color, it fails all tests means it is strictly less powelful than 1-WL test.
We can conclude than since GraphSage uses row normalized adjacency, it cannot have the degree of the vertices, it cannot tell the differences between two graphs if their sample distribution of vertex degrees are different. 
\end{proof}

\begin{theorem}
  \label{Th:thsage2}
GraphSage which uses full sampling and mean aggregator in \cite{hamilton2017sage}, has exactly the same power with 1-WL, if the vertices are initialized by their degrees with $H^{(0)}=A{\bf1},~H'^{(0)}=A'{\bf1}$.
\end{theorem}
\begin{proof}
%To make GraphSage more powerful, the degree of the nodes should be given as initial node color. 
1-WL equivalent graphs needs to meet conditions in Eq. \ref{eq:th1e1} for any initialization function $f(.)$. If we assume to initialize vertices by $H^{(0)}=(A{\bf 1})^{-1}$ and $H'^{(0)}=(A'{\bf 1})^{-1}$, for $t=0$, we have following condition for 1-WL test;
\begin{equation}
  \label{sageprof21}
  (A{\bf 1})^{-1}=\Pi (A'{\bf 1})^{-1}
\end{equation}
If we put the vector on to the diagonal of the matrix, it yields following;
\begin{equation}
  \label{sageprof22}
  diag(A{\bf 1})^{-1}=\Pi diag(A'{\bf 1})^{-1} \Pi^\top
\end{equation}
If we initialize the vertex color by their degree as $H^{(0)}=A{\bf 1}$ and $H'^{(0)}=A'{\bf 1}$, the output colors of second support of GraphSage become $H^{(1)}=\tilde{A}A{\bf 1}$ and $H'^{(1)}=\tilde{A'}A'{\bf 1}$. If the model decides that these graphs are isomorphic on this iterations, it should meet following condition;
\begin{equation}
  \label{sageprof23}
  \tilde{A}A{\bf 1} = \Pi \tilde{A'}A'{\bf 1}
\end{equation}
Since we can write row normalized adjacency by $\tilde{A}=diag(A{\bf 1})^{-1}A$, we can rewirte Eq. \ref{sageprof23} by following;
\begin{equation}
  \label{sageprof24}
  diag(A{\bf 1})^{-1}AA{\bf 1} = \Pi diag(A'{\bf 1})^{-1}A'A'{\bf 1}
\end{equation}
Using Eq.\ref{sageprof22}, since $\Pi$ is orthogonal, we can write $diag(A'{\bf 1})^{-1}=\Pi^\top diag(A{\bf 1})^{-1} \Pi$ and put it in Eq.\ref{sageprof24} as follows;
\begin{equation}
  \label{sageprof25}
  diag(A{\bf 1})^{-1}AA{\bf 1} = \Pi ~\Pi^\top diag(A{\bf 1})^{-1}\Pi A'A'{\bf 1}
\end{equation}
Since $\Pi ~\Pi^\top =I$ and $AA{\bf 1}=\Pi A'A'{\bf 1}$ for 1-WL in Eq.\ref{eq:th1e1}, we can obtain followings which shows both side is equal.
\begin{equation}
  \label{sageprof26}
  diag(A{\bf 1})^{-1}AA{\bf 1} =  diag(A{\bf 1})^{-1}\Pi A'A'{\bf 1}
\end{equation}
This shows that if the graphs are 1-WL equivalent, using row normalizing of adjacency instead of adjacency, does not change to being 1-WL equivalent. Since the GraphSage uses row normalized adjacency, we can conclude that they have exactly the same power. 
\end{proof}


\begin{theorem}
  \label{Th:thgcn}
GCN defined in \cite{kipf16:_semi} is not more powerful than 1-WL.
\end{theorem}
\begin{proof}
GCN uses single convolution support in Eq. \ref{eq:mpgnn} which is $C^{(1)}=(D+I)^{-0.5}(A+I)(D+I)^{-0.5}$ where $D$ is diagonal degree matrix \cite{kipf16:_semi}. To show that GCN is not more powerful than 1-WL, we should show that when 1-WL fails, GCN fails as well. Diagonal degree matrices can be written by $D=diag(A{\bf1})$ and $D'=diag(A'{\bf1})$ for both two graph's adjacency $A$ and $A'$. If 1-WL fails to distinguish this two non-isotropic graphs, then $A^t{\bf1}=\Pi A'^t{\bf1}$ must meet (Theorem~\ref{Th:th1}). Thus it yields following;
\begin{equation}
  \label{gcnproof1}
diag(A^t{\bf1})=\Pi diag(A'^t{\bf1}) \Pi^{\top}
\end{equation}
Since $\Pi$ is a permutation matrix (also orthogonal) we can write that $I=\Pi I \Pi^\top$ and add identity matrix both side of Eq. \ref{gcnproof1} as follows;
\begin{equation}
  \label{gcnproof2}
  \begin{split}
diag(A^t{\bf1})+I=\Pi diag(A'^t{\bf1}) \Pi^{\top} + \Pi I \Pi^\top \\
diag(A^t{\bf1}+{\bf1})=\Pi diag(A'^t{\bf1}+{\bf1}) \Pi^\top
\end{split}
\end{equation}
Since the matrices is diagonal, the power effects on element-wise on diagonal which yields following;
\begin{equation}
  \label{gcnproof3}
diag(A^t{\bf1}+{\bf1})^{-0.5}=\Pi diag(A'^t{\bf1}+{\bf1})^{-0.5} \Pi^\top
\end{equation}





the new color of vertex in iteration $t=1$ can be written by;
\begin{equation}
  \label{gcnproof}
        \begin{split}
H^{(1)}=diag(A{\bf1}+{\bf1})^{-0.5}A diag(A{\bf1}+{\bf1})^{-0.5}{\bf1}\\ +diag(A{\bf1}+{\bf1})^{-1}{\bf1} \\
 H'^{(1)}=diag(A'{\bf1}+{\bf1})^{-0.5}(A'+I)diag(A'{\bf1}+{\bf1})^{-0.5}{\bf1}
\end{split}
\end{equation}


and  respectively for two graphs. 
 
 
 \end{proof}

==> MNPPbeyondWL1_old.tex <==
\section{MPNN Beyond 1-WL}

Because of having the same memory and computational complexity and also similarity between Eq.\ref{eq:spat} and Eq.\ref{eq:wl1}, there is a consensus that all message passing GNN has equivalent power of 1-WL test. However, in this section, we theoretically show that some GNN is less powerful than 1-WL, some is strictly more powerful than 1-WL and also a way of breaking 1-WL limit to be able to have 3-WL (2-FWL) equivalent of Message Passing GNN. 

We call two graphs $G$ and $G'$ k-WL (or FWL) equivalent if they are indistinguishable by k-WL (or FWL) and shown by $G\equiv_{k-WL}G'$.
Since our analysis is limited for 1-WL and 3-WL (or 2-FWL) there is two options which are $G\equiv_{1-WL}G'$ and $G\equiv_{3-WL}G'$ (or $G\equiv_{2-FWL}G'$).

In our theoretical analysis, we consider the given two undirected graphs have the same number of featureless nodes and edges which is the most difficult case to test graph isomorphism.

\begin{theorem}
  \label{Th:th1}
Let $A,A' \in \{0,1\}^{n \times n}$ are the adjacency matrices of two undirected graphs consist of monochromatic nodes and edges. If they are 1-WL equivalent, there is a permutation matrix $\Pi \in \{0,1\}^{n \times n}$ which consist of single 1 in each rows and cols that meets following two constraints.
\begin{equation}
  \label{eq:th1e1}
  H^{(t)}=\Pi H'^{(t)}, ~~AH^{(t)}=\Pi A'H'^{(t)},  %\rightarrow
  %\sigma(A H^{(t)})=\Pi \sigma(A'H'^{(t)}), 
  ~~ \forall t \in N
\end{equation}
where $H^{(t)}=A H^{(t-1)},H'^{(t)}=A' H'^{(t-1)} \in \mathbb{R}^n$ is colors of vertices at iteration $t$, may be initialized by $H^{(0)}={\bf1}$.
\end{theorem}
\begin{proof}
If we simplify Eq \ref{eq:wl1} by using sum %followed by injective element-wise function
for order invariant set operator $\{.\}$, the update can be written by $H^{(t+1)} = \left( H^{(t)}~ |A H^{(t)} \right)$. For another graph, we can write it as $H'^{(t+1)} = \left( H'^{(t)}~ |A' H^{(t)} \right)$. According to definition of WL test, if two graphs are 1-WL equivalent, their node color histograms should be same at iteration $t+1$ thus, $hist\left( H^{(t)}~ |A H^{(t)} \right) = hist\left( H'^{(t)}~ |A' H'^{(t)} \right)$. If the histogram of two sets are equal, it means there is a permutation which rearrange one and get another. It means there is at least one $\Pi \in \{0,1\}^{n \times n}$ that meets  $\left( H^{(t)}~ |A H^{(t)} \right))= \Pi \left( H'^{(t)}~ |A' H'^{(t)} \right)$. Since $|$ is the concatenation operator, both parts of the equation should be equal independently under the same $\Pi$ permutation matrix. Thus , we can obtain Eq \ref{eq:th1e1}. If this constraint is met, the new color of the vertices are calculated and Eq.\ref{eq:th1e1} checks again. For new color calculation, we do not need to keep previous colors by $H^{(t)}$ and $H'^{(t)}$. Because they have the same color under the same permutation matrix by $AH^{(t)}$ and $A'H'^{(t)}$. It just have effect on elongate the color representation. Thus we can remove it as a part of relabelling process in 1-WL algorithm. The update needs to be $H^{(t+1)}=A H^{(t)},H'^{(t+1)}=A' H'^{(t)}$
\end{proof}

If the graphs are not 1-WL equivalent, at some $t$ iteration, Eq.\ref{eq:th1e1} does not meet. To compare any GNN's theoretical power with 1-WL, we should theoretically explain the constraints that GNN makes decision on equivalent, then find a situation where one concludes they are equivalent, but another not.

In order to analyse the theoretical power of GNN in terms of ability on distinguish non-isomorphic pairs of graphs, we can neglected the trainable parameters $W$ (assume $W=I$) and element-wise injective non-linearity $\sigma(.)$ (assume $\sigma(x)=x$) in Eq.\ref{eq:mpgnn}, since whatever they are, they cannot make any differences between graphs new embedding if the rest of them are the same ($H^{(t)}=\Pi H'^{(t)} \rightarrow  \sigma(W.H^{(t)})=\Pi \sigma(W.H'^{(t)})$). Thus new representation of the vertex color can be defined by $H^{(t+1)} =  \sum_s C^{(s)} H^{(t)}$ for GNN. For sake of simplicity, we can evaluate each convolution support independently for multi-support GNN case. If ever one support has ability to distinguish some pair of graphs, the model has that ability because of adding each supports embeddings to obtain final embeddings. 

\begin{theorem}
  \label{Th:thmlp}
Graph agnostic Neural Network named MLP cannot distinguish any pair of non-isomorphic graphs which can be identified by 1-WL at iteration $t>0$. Thus, MLP is strickly less powerful that 1-WL.
\end{theorem}
\begin{proof}
We can use MLP in order to make baseline if the structural information has effect to the problem target or not. In general framework in Eq. \ref{eq:mpgnn} we can define MLP by single convolution supports as it is $C^{(1)}=I$. To be equivalent according to MLP is to meet following constraint.

\begin{equation}
  \label{eq:thmlp}
  H^{(t)}=\Pi H'^{(t)}, ~~IH^{(t)}=\Pi I H'^{(t)}, ~~ \forall t \in N
\end{equation}

Since $H^{(t)}=IH^{(t)}$, actually second constraints does not say anything. It means, if the first constraint meet in Eq.\ref{eq:th1e1} but second not that 1-WL concludes that they are not isomorphic, still MLP's constraints meet (because first constraints of 1-WL is the same to both constraints of MLP) yields that MLP concludes they are isomorphic. Thus we can conclude that MLP is strictly less powerful than 1-WL. MLP can identify non-isomortphic graphs if they can be distinguishable by the given initial colors at iteration $t=0$ in 1-WL.
\end{proof}
\begin{theorem}
  \label{Th:thsage}
GraphSage which uses full sampling and mean aggregator in \cite{hamilton2017sage}, cannot distinguish any pair of non-isomorphic graphs, whose initial color is monochromatic. Thus, GraphSage is strickly less powerful that 1-WL.
\end{theorem}
\begin{proof}
In literature GraphSage method has was proposed to sample neighborhood and aggregate the neighborhood contribution by mean operator or LSTM in \cite{hamilton2017sage}. Since we restrict the method using full sampling and mean aggregator, we can define GraphSage by general framework in Eq.\ref{eq:mpgnn} while two convolution supports are identity matrix $C^{(1)}=I$ and row normalized adjacency matrix $C^{(2)}=\tilde{A}$. Theorem~\ref{Th:thmlp} shows that $C^{(1)}=I$ is nothing but just comparing initial vertex color. So we can just consider $C^{(2)}=\tilde{A}$. Thus constraints of GraphSage will be as follows;
\begin{equation}
  \label{eq:thsage1}
  H^{(t)}=\Pi H'^{(t)}, ~~\tilde{A}H^{(t)}=\Pi \tilde{A'} H'^{(t)}, ~~ \forall t \in N
\end{equation}
When we start by monochromatic vertex color as $H^{(0)}=H'^{(0)}={\bf1}$, since the row normalized adjacency meets $\tilde{A}{\bf1}=\tilde{A'}{\bf1}={\bf1}$, second constraint will always meet, even though the case where 1-WL's second constraint does not meet. %Thus we can conclude that if the GraphSage starts with monochromatic vertex color, it fails all tests means it is strictly less powelful than 1-WL test.
We can conclude than since GraphSage uses row normalized adjacency, it cannot have the degree of the vertices, it cannot tell the differences between two graphs if their sample distribution of vertex degrees are different. 
\end{proof}

\begin{theorem}
  \label{Th:thsage2}
GraphSage which uses full sampling and mean aggregator in \cite{hamilton2017sage}, has exactly the same power with 1-WL, if the vertices are initialized by their degrees with $H^{(0)}=A{\bf1},~H'^{(0)}=A'{\bf1}$.
\end{theorem}
\begin{proof}
%To make GraphSage more powerful, the degree of the nodes should be given as initial node color. 
1-WL equivalent graphs needs to meet conditions in Eq. \ref{eq:th1e1} for any initialization function $f(.)$. If we assume to initialize vertices by $H^{(0)}=(A{\bf 1})^{-1}$ and $H'^{(0)}=(A'{\bf 1})^{-1}$, for $t=0$, we have following condition for 1-WL test;
\begin{equation}
  \label{sageprof21}
  (A{\bf 1})^{-1}=\Pi (A'{\bf 1})^{-1}
\end{equation}
If we put the vector on to the diagonal of the matrix, it yields following;
\begin{equation}
  \label{sageprof22}
  diag(A{\bf 1})^{-1}=\Pi diag(A'{\bf 1})^{-1} \Pi^\top
\end{equation}
If we initialize the vertex color by their degree as $H^{(0)}=A{\bf 1}$ and $H'^{(0)}=A'{\bf 1}$, the output colors of second support of GraphSage become $H^{(1)}=\tilde{A}A{\bf 1}$ and $H'^{(1)}=\tilde{A'}A'{\bf 1}$. If the model decides that these graphs are isomorphic on this iterations, it should meet following condition;
\begin{equation}
  \label{sageprof23}
  \tilde{A}A{\bf 1} = \Pi \tilde{A'}A'{\bf 1}
\end{equation}
Since we can write row normalized adjacency by $\tilde{A}=diag(A{\bf 1})^{-1}A$, we can rewirte Eq. \ref{sageprof23} by following;
\begin{equation}
  \label{sageprof24}
  diag(A{\bf 1})^{-1}AA{\bf 1} = \Pi diag(A'{\bf 1})^{-1}A'A'{\bf 1}
\end{equation}
Using Eq.\ref{sageprof22}, since $\Pi$ is orthogonal, we can write $diag(A'{\bf 1})^{-1}=\Pi^\top diag(A{\bf 1})^{-1} \Pi$ and put it in Eq.\ref{sageprof24} as follows;
\begin{equation}
  \label{sageprof25}
  diag(A{\bf 1})^{-1}AA{\bf 1} = \Pi ~\Pi^\top diag(A{\bf 1})^{-1}\Pi A'A'{\bf 1}
\end{equation}
Since $\Pi ~\Pi^\top =I$ and $AA{\bf 1}=\Pi A'A'{\bf 1}$ for 1-WL in Eq.\ref{eq:th1e1}, we can obtain followings which shows both side is equal.
\begin{equation}
  \label{sageprof26}
  diag(A{\bf 1})^{-1}AA{\bf 1} =  diag(A{\bf 1})^{-1}\Pi A'A'{\bf 1}
\end{equation}
This shows that if the graphs are 1-WL equivalent, using row normalizing of adjacency instead of adjacency, does not change to being 1-WL equivalent. Since the GraphSage uses row normalized adjacency, we can conclude that they have exactly the same power. 
\end{proof}


\begin{theorem}
  \label{Th:thgcn}
GCN defined in \cite{kipf16:_semi} is not more powerful than 1-WL.
\end{theorem}
\begin{proof}
GCN uses single convolution support in Eq. \ref{eq:mpgnn} which is $C^{(1)}=(D+I)^{-0.5}(A+I)(D+I)^{-0.5}$ where $D$ is diagonal degree matrix \cite{kipf16:_semi}. To show that GCN is not more powerful than 1-WL, we should show that when 1-WL fails, GCN fails as well. Diagonal degree matrices can be written by $D=diag(A{\bf1})$ and $D'=diag(A'{\bf1})$ for both two graph's adjacency $A$ and $A'$. If 1-WL fails to distinguish this two non-isotropic graphs, then $A^t{\bf1}=\Pi A'^t{\bf1}$ must meet (Theorem~\ref{Th:th1}). Thus it yields following;
\begin{equation}
  \label{gcnproof1}
diag(A^t{\bf1})=\Pi diag(A'^t{\bf1}) \Pi^{\top}
\end{equation}
Since $\Pi$ is a permutation matrix (also orthogonal) we can write that $I=\Pi I \Pi^\top$ and add identity matrix both side of Eq. \ref{gcnproof1} as follows;
\begin{equation}
  \label{gcnproof2}
  \begin{split}
diag(A^t{\bf1})+I=\Pi diag(A'^t{\bf1}) \Pi^{\top} + \Pi I \Pi^\top \\
diag(A^t{\bf1}+{\bf1})=\Pi diag(A'^t{\bf1}+{\bf1}) \Pi^\top
\end{split}
\end{equation}
Since the matrices is diagonal, the power effects on element-wise on diagonal which yields following;
\begin{equation}
  \label{gcnproof3}
diag(A^t{\bf1}+{\bf1})^{-0.5}=\Pi diag(A'^t{\bf1}+{\bf1})^{-0.5} \Pi^\top
\end{equation}





the new color of vertex in iteration $t=1$ can be written by;
\begin{equation}
  \label{gcnproof}
        \begin{split}
H^{(1)}=diag(A{\bf1}+{\bf1})^{-0.5}A diag(A{\bf1}+{\bf1})^{-0.5}{\bf1}\\ +diag(A{\bf1}+{\bf1})^{-1}{\bf1} \\
 H'^{(1)}=diag(A'{\bf1}+{\bf1})^{-0.5}(A'+I)diag(A'{\bf1}+{\bf1})^{-0.5}{\bf1}
\end{split}
\end{equation}


and  respectively for two graphs. 
 
 
 \end{proof}

==> WLdefinition.tex <==
\section{Weisfeiler-Lehman Test}

The universality of a GNN is based on its ability to embed two non-isomorphic graphs to distinct points in the target feature space. A model which can distinguish all pairs of non-isomorphic graphs is a universal approximator. Since it is not known if the graph isomorphism problem can be solved in polynomial time or not, this problem is neither NP-complete nor P, but NP-intermediate \cite{takapoui2016linear}. One of the oldest but prominent polynomial approach is the Weisfeiler-Lehman Test (abbreviated WL-test) which gives 
%named WL test gives
sufficient but not enough evidence. WL test can be extended by taking into account higher order of node tuple within the iterative process. These extensions are denoted as $k$-WL test, where $k$ is equals to the order of the tuple. It is important to mention that an higher order of tuple leads to a better ability to distinguish two non-isomorphic graphs (with the exception for $k=2$) ~\cite{arvind2020weisfeiler}.

%enumerated by the order of node tuple used in the iteration such as 1-WL, 2-WL,..,k-WL where the one is more powerful than its ancestor in terms of ability to distinguish two non-isomorphic graphs \cite{arvind2020weisfeiler}.

The 1-WL test, known as vertex coloring, starts with the given initial color of nodes if available (unless assume all nodes are monochromatic, so all nodes color is the same, $H_v^{(0)}=1$) and updates the color by the following iteration:
\begin{equation}
  \label{eq:wl1}
  H_v^{(t+1)} =\sigma \left( H_v^{(t)}~ |\left\{ H_u^{(t)} : u \in \mathcal{N}(v) \right\} \right),
\end{equation}
where $H_v^{(t)}$ is the color of vertex $v$ at iteration $t$, $\mathcal{N}(v)$ is the set of neighbours of vertex $v$, the concatenation operator is represented by $|$ and order invariant set can be shown by $\{.\}$, which is % where we
generally implemented %it
by stacking all colors in the set and sorting them alphabetically. To avoid the new color of vertex become bigger after each iteration, $\sigma(.)$ function performs the recoloring step where it assigns a new color identifier to the every new created unique color. The test should be done in parallel for two graphs and iterative process is stopped when the histograms are not changing between two iterations.
%of color is not changing between two iterations. and color histograms are compared after each iteration.
% after every iteration histogram of vertex color should be compared.
If the histograms are different in any iteration we can conclude that the graphs are not isomorphic. Conversely, two same histograms may be computed even for non-isomorphic graphs.
%Even after new iteration, the colors of the nodes do not change and still the histograms are the same, we can end the iteration however cannot be sure that these two graphs are not isomorphic. 

Higher order WL tests use the same algorithm while their color update schema is slightly different. 2-WL test uses second order tuple of nodes (all ordered pairs of nodes), thus it needs $\mathbf{H} \in \mathbb{R}^{n \times n}$ matrix, where initial colors have two more colors than initial vertex colors as defined by:
\begin{equation}
  \label{wl2initial}
  \mathbf{H}_{v,u}^{(0)} = \left\{
        \begin{array}{l@{\text{ ~~~~if~ }}l}
            H_v^{(0)} & v = u \\           
            edge & u \in \mathcal{N}(v) \\  
            nonedge & u \not\in \mathcal{N}(v) \\
        \end{array}
    \right. 
\end{equation}
Then the iteration uses following schema where $[n]$ is the set of node identifiers.
\begin{equation}
  \label{eq:wl2}
  \mathbf{H}_{v,u}^{(t+1)} =\sigma \left( \mathbf{H}_{v,u}^{(t)}~ |\left\{ \mathbf{H}_{v,k}^{(t)} : k \in [n] \right\} |\left\{ \mathbf{H}_{k,u}^{(t)} : k \in [n] \right\} \right),
\end{equation}
Although for $k\geq2$, $(k+1)$-WL $>$ $(k)$-WL, it is not true for $k=1$, thus given 2-WL in Eq.\ref{eq:wl2} is no more powerful than 1-WL in \ref{eq:wl1} \cite{maron2019provably}. To clarify this point,
Folkore WL (FWL) test is defined such as 1-WL=1-FWL, but for $k \geq 2$, we have $(k+1)$-WL $\approx$ $(k)$-FWL~\cite{maron2019provably}.
%In this point, there is another version of WL named Folklore WL (FWL) which is exactly the same for $k=1$, thus 1-WL=1-FWL but for $k\geq2$, $(k+1)$-WL $\approx$ $(k)$-FWL \cite{maron2019provably}.
The iteration process of 2-FWL can be shown by following equation;
\begin{equation}
  \label{eq:fwl2}
  \mathbf{H}_{v,u}^{(t+1)} =\sigma \left( \mathbf{H}_{v,u}^{(t)}~ |\left\{ \left( \mathbf{H}_{v,k}^{(t)} | \mathbf{H}_{k,u}^{(t)} \right) : k \in [n]  \right\} \right),
\end{equation}

In literature, there is a conflict to use the order of the WL test. Some papers use defined WL test order in Eq.~\ref{eq:wl1} and Eq.~\ref{eq:wl2} \cite{123lehmango, maron2019provably} but some others use FWL order under the name of WL such as in \cite{abboud2020surprising,arvind2020weisfeiler,takapoui2016linear}. In this paper, we explicitly mention both WL and FWL equivalent such as 3-WL (or 2-FWL) to alleviate ambiguities.


==> characterization.tex <==
\section{Characterization of WL Test}

In order to better understand the capability of WL tests, some papers attempt to characterize these tests using a first order logic \cite{immerman1990describing,barcelo2019logical}. If graphs are represented by their adjacency matrix, assuming undirected graphs with non-chromatic edges and nodes, two graphs adjacency matrices denoted $A_G$ and $A_H$ are said k-WL (or k-FWL) equivalent, denoted by $A_G\equiv_{k-WL}A_H$, if the corresponding graphs are indistinguishable by k-WL (or k-FWL). %Since our analysis is limited to 1-WL and 3-WL (or 2-FWL) we use the notations $A_G\equiv_{1-WL}A_H$ and $A_G\equiv_{3-WL}A_H$ (or $A_G\equiv_{2-FWL}A_H$). 

%\begin{remark}
% \label{rm:rm1}
%It was shown that 1-WL can be characterized by first order logic restricted by 2 variables named $C_2$, thus $A_G\equiv_{1-WL}A_H \leftrightarrow A_G\equiv_{C_2}A_H$. While 3-WL (or 2-FWL) characterized by 3 variables logic named $C_3$, thus $A_G\equiv_{3-WL}A_H \leftrightarrow A_G\equiv_{2-FWL}A_H \leftrightarrow A_G\equiv_{C_3}A_H$ \cite{cai1992optimal,immerman1990describing}.  
%\end{remark}


%Recently the approach based on new created Matrix Language (MATLANG) comes out \cite{geerts2020expressive,brijder2019expressive}. They defined a new Matrix Languages which has different allowed operations in their dictionary and they did explicit connection from these specific dictionaries to the 1-WL and 3-WL tests. Beside they proposed many different fragment of operations (dictionaries) whose expressive powers are vary.

Recently \cite{brijder2019expressive,geerts2020expressive} propose a new Matrix Languages called MATLANG with a dictionary of different allowed operations and make some explicit connections between specific dictionaries and the 1-WL and 3-WL tests. This way, they propose many different fragments of operation (dictionaries) whose expressive powers vary.

\begin{definition}
$ML(\mathcal{L})$ is a matrix language which with an allowed operation set $\mathcal{L}=\{op_1,\dots op_n\}$ where $op_n \in \{.,+,^\top,diag,tr,{\bf1},\circ, \times,f\}$. The possible operations are matrices multiplication and addition, matrix transpose, vector diagonalization, matrix trace computation, column vector full of 1, element-wise matrix multiplication, matrix/scalar multiplication and element-wise custom function operating on scalars or vectors.
\end{definition}

\begin{definition}
$e(X) \in \mathbb{C}$ is a sentence in $ML(\mathcal{L})$ which consist of any possible consecutive operations in $\mathcal{L}$, operating on a given matrix $X$ and resulting in a complex scalar value. 
\end{definition}

As an example, $e(X)={\bf1}^{\top}X^2{\bf1}$ is a sentence of $ML(\mathcal{L})$ with $\mathcal{L}=\{.,^\top,{\bf1}\}$ which gives the sum of all element in square of matrix $X$. In the following, we are interested in three languages with operation sets $\mathcal{L}_1,\mathcal{L}_2$ and $\mathcal{L}_3$ which have been used for characterizing the WL-test in \cite{geerts2020expressive}. These results are given by the following remarks :

\begin{remark}
 \label{rm:rm2}
Two graphs are indistinguishable by the 1-WL test if and only if their adjacency matrices are indistinguishable by any sentences in $ML(\mathcal{L}_1)$ with $\mathcal{L}_1=\{.,^\top,{\bf1},diag\}$. Hence, all possible sentences in $\mathcal{L}_1$ are the same for 1-WL equivalent adjacency matrices. Thus, $A_G\equiv_{1-WL}A_H \leftrightarrow A_G\equiv_{ML(\mathcal{L}_1)}A_H$. (see Theorem 7.1 in \cite{geerts2020expressive})
\end{remark}

\begin{remark}
 \label{rm:rm3}
$ML(\mathcal{L}_2)$ with $\mathcal{L}_2=\{.,^\top,{\bf1},diag,tr\}$ is strictly more powerful than $\mathcal{L}_1$, i.e. than the 1-WL test, but less powerful than the 3-WL test. (see Theorem 7.2~Example 7.3 in  \cite{geerts2020expressive})
\end{remark}


\begin{remark}
 \label{rm:rm5}
Two adjacency matrices are indistinguishable by the 3-WL test if and only if they are indistinguishable by any sentences in $ML(\mathcal{L}_3)$ with  $\mathcal{L}_3=\{.,^\top,{\bf1},diag,tr,\circ\}$. Thus, $A_G\equiv_{3-WL}A_H \leftrightarrow A_G\equiv_{ML(\mathcal{L}_3)}A_H$. (see Theorem 9.2 in \cite{geerts2020expressive})
\end{remark}


\begin{remark}
 \label{rm:rm4}
Enriching the operation set by $\mathcal{L}^+=\mathcal{L} \cup \{ +,\times,f\}$ where $\mathcal{L} \in (\mathcal{L}_1,\mathcal{L}_2,\mathcal{L}_3$) do not improve the expressive power of the language. Thus, $A_G\equiv_{ML(\mathcal{L})}A_H \leftrightarrow A_G\equiv_{ML(\mathcal{L}^+)}A_H$. (see Proposition~7.5 in \cite{geerts2020expressive})
\end{remark}



==> designpowerfulMPNN.tex <==
\section{How Powerful is MPNN?}

This section presents some results about the theoretical expressive power of state of the art MPNNs. Those results have been derived using using the MATLANG language  \cite{geerts2020expressive} and more precisely the remarks of the preceding section. Proofs of the theorems are given in appendix \ref{section:app_prof}.  

\begin{theorem}
\label{th:thmpnn}
The graphs MPNNs GCN, GAT, GraphSage and GIN cannot go further than operations in $\mathcal{L}_1^+$. They are not more powerful than the 1-WL test.
\end{theorem}

The result has already been given in \cite{xu2018how} which proposes GIN-$\epsilon$ and show that it is the unique Graph MPNN which is provably as powerful as the 1-WL test, under the assumption that $\epsilon$ is an irrational number in order to make the graph readout function injective. 

Chebnet is also known not to be more powerful than the 1-WL test. However we the next theorem states that it is true if the maximum eigenvalues are the same for both graphs. For a pair of graph whose maximum eigenvalues are not equal, Chebnet is strictly more powerful than 1-WL test. 

\begin{theorem}
\label{th:chebnet}
Chebnet is more powerful than the 1-WL test if the Laplacian maximum eigenvalues of the graphs to be compared are not the same. Unless Chebnet is not more powerful than 1-WL.
\end{theorem}


%{\color{red}However, we did not find counter example that shows GIN is succeed to distinguish two non-isomorphic graphs to each other but not Graph MPNN such as Chebnet, GCN, GAT or SageGraph known as not powerful than 1-WL. Still, they might be less powerful than 1-WL test.}

Following theorem shows another prove of the studied Graph MPNN are not more powerful than 1-WL test in terms of graph isomorphism test.

\begin{theorem}
\label{th:thmpnn}
Well-known Graph MPNNs named GCN, GAT, GraphSage, GIN cannot go further than operations in $\mathcal{L}_1^+$, thus they are not more powerful than 1-WL test.
\end{theorem}

Chebnet is also known that it is not more powerful than 1-WL test. However we show in the next theorem that it is true if the maximum eigenvalues are the same. For the pair of graph whose maximum eigenvalue is not equal, Chebnet is strictly more powerful than 1-WL test. 

\begin{theorem}
\label{th:chebnet}
If the tested two graph's laplacien's maximum eignevalues are not the same, Chebnet produces outputs that sentences in  $\mathcal{L}_1^+$ do not. Thus, thus Chebnet is more powerful than 1-WL test in this case, unless it is not more powerful than 1-WL.
\end{theorem}
  

{\color{red} Can this example be shiflted in the appendix ? I mean, is it necessary for the following ?

\begin{figure}[ht]
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.6\columnwidth]{figures/decalin_bicyclopentyl.png}}
\caption{Decalin ($G$) and Bicyclopentyl ($H$) graphs are $\mathcal{L}_1$ and also 1-WL equivalent, but Chebnet can distinguish them.
}
\label{dec_bicyc}
\end{center}
\vskip -0.2in
\end{figure}

In Figure~\ref{dec_bicyc}, there are two sample graphs which are 1-WL equivalent and are generally used to show how MPNN fails to distinguish these two graphs. However, their normalized laplacien's maximum eigenvalues are 2 and 1.8418 respectively. It yields using just one layer Chebnet by second support and sum operation on graph readout layer, the outputs become ${\bf1}^{\top}C^{(2)}_{G}H^{(0)} \neq {\bf1}^{\top}C^{(2)}_{H}H^{(0)}$ where $H^{(0)}={\bf1}$ initial monochrome node features. Thus, Chebnet can project these two graphs to different points in feature space. Details can be found in Appendix~\ref{app2}.}

{\color{red} To be rephrased}

However, this fact does not give enough power to the model, since there are infinite number of 1-WL equivalent graphs whose maximum eigenvalues are the same. Beside, rest of the algorithms such as GCN, GIN, GAT, GraphSage can take this advantage easily by scaling their convolution support by $2/\lambda_{max}$.

As stated in the introduction, comparison with the WL-test is not the only way to characterize the expressive power of GNNs. Powerful GNN are also  expected to be able to count necessary substructures in a given graph for specific problems. With the following theorems, we show which matrix language is needed to be able to count the graphlets illustrated in Figure~\ref{substruct} which are called 3-star, triangle, tailed triangle and 4-cycle. 

\begin{figure}[ht]
%\vskip 0.2in
\begin{center}
\centerline{\includegraphics[width=0.8\columnwidth]{figures/substructure.jpg}}
\caption{Sample 4-vertex patterns. 3-star, triangle, tailed triangle and 4-cycle graphlets used in our analysis.
}
\label{substruct}
\end{center}
\vskip -0.2in
\end{figure}

\begin{theorem}
\label{th:star3}
3-stars graphlet can be countable by sentences in  $\mathcal{L}_1^+$.
\end{theorem}

\begin{theorem}
\label{th:triangle}
Triangle and 4-cycle graphlets can be countable by sentences in  $\mathcal{L}_2^+$.
\end{theorem}

\begin{theorem}
\label{th:tailed4cycle}
Tailed triangle graphlet can be countable by sentences in  $\mathcal{L}_3^+$.
\end{theorem}

According to above Theorems, 1-WL equivalent MPNN can only count 3-star pattern while 3-WL equivalent MPNN can count all studied graphlets. It was shown that if the MPNN has no appropriate convolution support ($A$), it cannot learn even node degrees well \cite{DehmamyBY19}. That is why we assume the node degrees are given as a node features in order to do fair comparison. Since the number of 3-stars graphlet is a function of node degree and node degree is the uniue necessary feature that can be calculated by operation in $\mathcal{L}_1$ for 3-stars counting as shown in Appendix~\ref{section:prth3}, if the node degree is given as as input, the graph agnostic neural network MLP can also count it perfectly.

% Because, to calculate number of 3-stars we just need node degree from operations in $\mathcal{L}_1$ explained in Appendix~\ref{section:prth3}. So, if it is given as input, we just need to approximate combination function that can be done by MLP.

==> introductionv0.tex <==
{\color{red} In red : points to be discussed since I do not understand}

{\color{blue} In blue : modified sentences to be checked by you Muhammet and put it back in black if you are OK}
 

In the past few years, finding the best inductive bias for relational data represented as graphs has gained a lot of interest in the machine learning community. Node based message passing mechanisms relying on the graph structure, have given rise to the first generation of Graph Neural Networks (GNNs) called Message Passing Neural Network (MPNN). These algorithms spread each node features to the neighborhood nodes using trainable weights. These weights can be shared with respect to the distance between nodes \cite{defferrard16:_convol_neural_networ_graph_fast}, to the connected nodes features \cite{velivckovic2017graph} and/or to edge features \cite{bresson2017residual}. {\color{blue}When considering sparse graphs, the memory and computational complexity of such approaches are linear with respect to number of nodes. Thus, these algorithms are feasible for large sparse graphs.}

% OK for §1

Despite this interesting computational property, it has been shown recently that these methods are not universal approximator {\color{blue} since they embed two non-isomorphic graphs to exactly the same point if these two graphs are not distinguishable by the first order Weisfeiler-Lehman test known as 1-WL \cite{xu2018how}}. {\color{blue}Thus, from a theoretical expressive power point of view, node based message passing algorithms are not more powerful than 1-WL.} {\color{red} Not just full solution of graph isomorphism but also many combinatorial problems on graph cannot be solved MPNN \cite{satonips}}.  

{\color{blue} In \cite{universalmaron19a,NIPS2019_8931}, it has been proved that to reach universal approximation, higher order relations are needed. However, using such relations makes both memory and computational complexities grown exponentially}. Thus, it is not feasible to have universal approximation models in practice. That is why most recent researches focused on proposing GNNs with a theoretical power according to WL test order as high as possible and a  complexity as low as possible. 

In this context, some powerful models which are equivalent to 3-WL were proposed. For instance, \cite{maron2019provably} proposed {\color{red}the model that mimics the} second order Folklore WL test (2-FWL) which is equivalent to 3-WL, \cite{123lehmango} uses message passing between 1,2 and 3 order node tuple hierarchically, thus meeting the 3-WL expressive power. However both memory and time complexity of these methods are higher. 

Alternatively, to keep the complexity linear, some researches proposed to increase the theoretical expressive power of MPNN using enhanced node features by random noise \cite{abboud2020surprising,sato2020random} or unique label \cite{murphy19a} in order to have ability to distinguish two graphs which the 1-WL fails. A very recent research extracts some features in preprocessing step which cannot be extracted by MPNN, thus they improve the expressive power of MPNN \cite{bouritsas2020improving}. However, we do not think these solutions are the proper way because it needs massively training samples and slow convergence to learn the dynamic of the structure by noise or given node ids and needs many handcrafted features which needs domain expertise and infinite number of possible features selection.  

Having theoretically more powerful model makes it closer to universal approximation. However, it does not mean that the generalization ability has to be increased simultaneously. Since most of the realistic problems where graphs are given with many either continuous or discrete node/edge feature, there is almost no pair of graph which is not distinguishable by 1-WL. In addition, theoretically more powerful methods use non-local updates that is against the one of the most important inductive bias in Euclidean learning named locality principle \cite{battaglia2018relational}. These may explain why theoretical powerful methods cannot outperformed MPNN on many downstream tasks where the results are reported in \cite{dwivedi2020benchmarking}.

On the other hand, it does not mean that 1-WL equivalent GNN is enough since we have known that they cannot extract some structural features such as number of cycles or triangles \cite{arvind2020weisfeiler,chen2020can,bouritsas2020improving} which are informative for some social or chemical graphs. In addition to have theoretical powerful model, some researches shows that we need to pay attention to the spectral ability of the model where vast majority of the MPNNs actually work as low-pass filters \cite{balcilar2021analyzing}. 

To overcome all those mentioned problems of GNN, here we propose to design graph convolution in spectral domain by custom non-linear function except integer power of eigenvalues and mask the convolution support by desired length of receptive field. In this way, we have spatially local updates process, linear memory and computational complexity (except eigendecomposition in preprocessing step), enough spectral ability and also theoretically as powerful as 3-WL model. In our experiments, we show that proposed model is able to count some substructures that 1-WL equivalent MPNN cannot, its spectral ability is enough to produce various kind of spectral component in the output while vast majority of the GNNs includes higher order WL equivalents models do not, it can distinguish the pair of graphs which cannot be distinguishable by 1-WL equivalent MPNN and thank to the sparse matrix multiplication it has linear time complexity except the eigendecompostion in preprocessing step.
